Compressing Long Context into Answer-Aligned Memory Embeddings for LLM Inference

Large language model (LLM) inference is constrained by the quadratic scaling of self-attention and the linear scaling of the KV cache, increasing latency, energy consumption, and GPU memory demand as context length scales. Existing soft-compression methods either lack query-guided memory selection at inference time, train without answer-targeted supervision, or couple compression tightly to a specific decoder architecture. We propose a Context-to-Answer-Aligned Memory Compression (CMC) framework, which compresses long input contexts into compact Context Memory Embeddings (CMEs) aligned to any frozen decoder's embedding space, reducing inference costs without modifying decoder weights. CMC introduces a two-tier KV cache that combines question-guided CME selection with a local context window, and trains the compressor with answer-targeted distillation from a frozen LLM. Experiments across nine encoder-decoder combinations and four QA benchmarks show that CMC consistently outperforms the baseline, achieving up to 7.3 EM and 4.0 F1 point gains on SQuAD, while reducing inference time and energy consumption by up to 20% and peak reserved GPU memory by up to 50% at 3,000 generation tokens. Ablation studies confirm that each architectural component and training objective contributes to the performance.

==> accuracy-comparison-imdb.tex <==
\begin{axis}[
    ybar=.05cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=5.7cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.08,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=89, 
    ylabel={$\mathbf{A}$  (\%)},
    %xlabel={Datasets},
    %symbolic x coords={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
    %xtick=data,
    xtick={1,2,3,4,5,6,7,8, 9, 10},
    %nodes near coords,
    ytick={89, 89.5, 90, 90.50, 91, 91.50, 92, 92.50},
    xticklabels={BERT-base, -LSTM,  RoBERTa-base, -GRU, GPT2, -GRU, DeepSeek-Coder, -LSTM, DeepSeek-R1, -BiGRU},
    x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=6pt,
    bar shift=0,
    %ymajorgrids=true,
    label style={font=\tiny},
    ]
%\addplot [draw=black, semithick, color=red, preaction={fill, red}, pattern=crosshatch dots, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.31) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.35)};  %  F1w Scores 

%\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)};  % A Scores 



\addplot [draw=blue, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white]  coordinates {(1,90.96)}; % BERT-base

\addplot  [draw=blue, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white]   coordinates {(2,91.32)}; % BERT-LSTM


\addplot [draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white] coordinates {(3,91.32)}; % RoBERTa-base

\addplot [draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white]coordinates {(4,92.60)}; % RoBERTa-GRU


\addplot  [draw=blue, color=blue, preaction={fill, blue}, semithick, pattern=grid, pattern color = white]  coordinates {(5,91.16)}; % GPT2

\addplot [draw=blue, color=blue, preaction={fill, blue}, semithick, pattern=grid, pattern color = white]   coordinates {(6,91.92)}; % GPT2-GRU




\addplot[draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white]coordinates {(7,89.60)}; % DS-Coder

\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(8,90.76)}; % DS-Coder-LSTM



\addplot[draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white]coordinates {(9,90.08)}; % DS-R1

\addplot [draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white] coordinates {(10,90.48)}; % DS-R1-BiGRU




%(BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)







%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

%\legend{$\mathbf{F1}_w$ Score, $\mathbf{A}$ Score}
\end{axis}
 


==> accuracy-comparison-sentiment140.tex <==
\begin{axis}[
    ybar=.05cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=5.7cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.08,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=77, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    %symbolic x coords={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
    %xtick=data,
    xtick={1,2,3,4,5,6,7,8, 9, 10},
    %nodes near coords,
    ytick={77, 78, 79, 80, 81, 82, 83},
    xticklabels={BERT-base, -GRU, RoBERTa-base, -GRU, GPT2, -BiLSTM, DeepSeek-Coder, -BiGRU, DeepSeek-R1, -LSTM},
    x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=6pt,
    bar shift=0,
    %ymajorgrids=true,
    label style={font=\tiny},
    ]
%\addplot [draw=black, semithick, color=red, preaction={fill, red}, pattern=crosshatch dots, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.31) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.35)};  %  F1w Scores 

%\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)};  % A Scores 



\addplot  [draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white] coordinates {(1,81.35)}; % BERT-base



\addplot  [draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white]   coordinates {(2,81.83)}; % BERT-GRU


\addplot [draw=black, color=Purple, preaction={fill, Purple}, semithick, pattern=grid, pattern color = white] coordinates {(3,82.17)}; % RoBERTa-base

\addplot [draw=black, color=Purple, preaction={fill, Purple}, semithick, pattern=grid, pattern color = white] coordinates {(4,82.32)}; % RoBERTa-GRU



\addplot   [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white]  coordinates {(5,81.18)}; % GPT2

\addplot  [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white]  coordinates {(6,80.97)}; % GPT2-BiLSTM



\addplot[draw=black, color=blue, preaction={fill, blue}, semithick, pattern=grid, pattern color = white] coordinates {(7,77.81)}; % DS

\addplot [draw=black, color=blue, preaction={fill, blue}, semithick, pattern=grid, pattern color = white] coordinates {(8,79.59)}; % DS-Coder-BiGRU


\addplot[draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white]coordinates {(9,78.47)}; % DS-R1

\addplot [draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white] coordinates {(10,80.44)}; % DS-R1-LSTM




%(BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)







%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

%\legend{$\mathbf{F1}_w$ Score, $\mathbf{A}$ Score}
\end{axis}
 


==> accuracy-comparison-twitter.tex <==
\begin{axis}[
    ybar=.05cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=5.7cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.08,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=74, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    %symbolic x coords={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
    %xtick=data,
    xtick={1,2,3,4,5,6,7,8, 9, 10},
    %nodes near coords,
    ytick={71, 72, 73, 74, 75, 76, 77, 78, 79, 80, 81},
    xticklabels={BERT-base, -BiLSTM,  RoBERTa-base, -BiLSTM, GPT2, -LSTM, DeepSeek-Coder, -LSTM, DeepSeek-R1, -BiLSTM},
    x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=6pt,
    bar shift=0,
    %ymajorgrids=true,
    label style={font=\tiny},
    ]
%\addplot [draw=black, semithick, color=red, preaction={fill, red}, pattern=crosshatch dots, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.31) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.35)};  %  F1w Scores 

%\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)};  % A Scores 



\addplot [draw=blue, color=teal, preaction={fill, teal}, semithick, pattern=grid, pattern color = white]  coordinates {(1,75.27)}; % BERT-base

\addplot [draw=blue, color=teal, preaction={fill, teal}, semithick, pattern=grid, pattern color = white]   coordinates {(2,79.37)}; % BERT-BiLSTM


\addplot [draw=black, color=Magenta, preaction={fill, Magenta}, semithick, pattern=grid, pattern color = white] coordinates {(3,79.78)}; % RoBERTa-base



\addplot [draw=black, color=Magenta, preaction={fill, Magenta}, semithick, pattern=grid, pattern color = white] coordinates {(4,80.74)}; % RoBERTa-BiLSTM



\addplot [draw=blue, color=blue, preaction={fill, blue}, semithick, pattern=grid, pattern color = white]   coordinates {(5,77.46)}; % GPT2

\addplot [draw=blue, color=blue, preaction={fill, blue}, semithick, pattern=grid, pattern color = white]   coordinates {(6,79.10)}; % GPT2-LSTM

\addplot [draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white] coordinates {(7,80.33)}; % DS

\addplot [draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white] coordinates {(8,80.60)}; % DS-LSTM



\addplot[draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white]coordinates {(9,79.37)}; % DS-R1

\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(10,79.51)}; % DS-R1-BiLSTM



%(BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)







%\addplot [draw=black, semithick, pattern=grid, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

%\legend{$\mathbf{F1}_w$ Score, $\mathbf{A}$ Score}
\end{axis}
 


==> accuracy_comparison.tex <==
\begin{axis}[
    ybar=.15cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    width=\linewidth,
    %width=6.8cm,
    height=5cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.40,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.15)},
    anchor=north, legend columns=-1},
    ymin=55, 
    ymax=90,
    ylabel={ Average Accuracy (\%)},
    %xlabel={Datasets},
    symbolic x coords={Commonsense, Code Understanding, Biomedical},
    xtick=data,
    %nodes near coords,
    ytick={10, 20, 30, 40, 50, 55, 60, 65, 70, 75, 80, 85,  90, 95, 100},
    %x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=15pt,
    %ymajorgrids=true,
    label style={font=\tiny},
    ]
%\addplot [draw=teal, semithick, pattern=horizontal lines, pattern color = teal] coordinates {(IMDb,91.12) (Twitter US Airline,78.83) (Sentiment140,81.83)};  % Macro F1-Score for 0.001

\addplot [draw=cyan, semithick, pattern=bricks, fill=cyan,  pattern color = blue] coordinates {(Commonsense,83.22) (Code Understanding,63.22) (Biomedical,88.21)};  % Macro F1-Score for 0.005

\addplot [draw=Salmon, semithick, pattern=crosshatch dots, fill=Salmon,  pattern color = red] coordinates {(Commonsense,84.33) (Code Understanding,67.03) (Biomedical,88.58)}; % Macro F1-Score for 0.01

%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

\legend{Baseline LLMs, LLM-RNN Models}
\end{axis}
 


==> accuracy_scores_SearchAlg.tex <==
\begin{axis}[
    ybar=.08cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=5.9cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.2,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.22)},
    anchor=north, legend columns=-2},
    ymin=90, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    symbolic x coords={RoBERTa, CodeBERT, CodeT5, CodeT5$^+$, DeepSeek-Coder},
    xtick=data,
    %nodes near coords,
    ytick={10, 20, 30, 40, 50, 60, 70, 80, 90, 91, 92, 93, 94, 95, 96, 97, 98, 99, 100},
    %x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=4pt,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
\addplot [draw=teal, semithick, pattern=grid, pattern color = teal] coordinates {(RoBERTa,93.44) (CodeBERT,93.59) (CodeT5, 94.40) (CodeT5$^+$, 95)};  % Macro F1-Score for 0.001

\addplot [draw=magenta, semithick, pattern=bricks,  pattern color = magenta] coordinates {(RoBERTa,93.55) (CodeBERT,94.01) (CodeT5, 95.12) (CodeT5$^+$, 96)};  % Macro F1-Score for 0.005

\addplot [draw=blue, semithick, pattern=crosshatch dots,  pattern color = blue] coordinates {(RoBERTa,93.44) (CodeBERT,93.82) (CodeT5, 94.17) (CodeT5$^+$, 96)}; % Macro F1-Score for 0.01

\addplot [draw=red, semithick, pattern=north west lines,  pattern color = red] coordinates {(RoBERTa,93.59) (CodeBERT,93.97) (CodeT5,94.86) (CodeT5$^+$, 96)}; % Macro F1-Score for 0.01

%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

\legend{LSTM, BiLSTM, GRU, BiGRU}
\end{axis}
 


==> accuracy_scores_SearchAlg_curve.tex <==

\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    %xlabel={$minSup$},
    ylabel={$\mathbf{A}$ (\%)},
    ylabel near ticks, ylabel shift={-5pt},
    width=\linewidth,
    width=5.9cm,
    height=4cm,
    grid,
    grid style={gray!50},
    grid=both,
    ymin=90,
    %xmin=0, xmax=13,
    %ymin=20, ymax=75,
    % xtick={0,20,40,60,80,100},
    ytick={90,91,92,93,94,95,96,97},
    %legend style={at={(axis cs:10,60)},anchor=south east},
    symbolic x coords={Base, LSTM, BiLSTM, GRU, BiGRU},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    ymajorgrids=true,
    grid style=solid,
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    legend style={at={(1.7,1.02)}, draw=none, anchor=south, legend columns=5},
    %legend style={at={(0.5,-0.20)},
    %legend style={draw=none},
    %anchor=north, legend columns=3},
]

%\addplot [mark=*, red, dashed] table[x=N,y=No_Sym] {data.dat};


\addplot[mark=otimes*, orange, solid, every mark/.append style={solid, fill=orange}]
    coordinates {
(Base,90.54)
(LSTM,93.44)
(BiLSTM,93.55)
(GRU,93.44)
(BiGRU,93.59)
    };
    \addlegendentry{RoBERTa}
    
\addplot[mark=square*, blue, solid, every mark/.append style={solid, fill=blue}]
    coordinates {
(Base,92.33)
(LSTM,93.59)
(BiLSTM,94.01)
(GRU,93.82)
(BiGRU,93.97)


    };
\addlegendentry{CodeBERT}

\addplot[mark=diamond*, red, solid, every mark/.append style={solid, fill=red}]
    coordinates {
(Base,93.61)
(LSTM,94.40)
(BiLSTM,95.12)
(GRU,94.17)
(BiGRU,94.86)
    };
\addlegendentry{CodeT5}

\addplot[mark=*, teal, solid, every mark/.append style={solid, fill=teal}]
    coordinates {
(Base,93.38)
(LSTM,95.00)
(BiLSTM,96.00)
(GRU,96.00)
(BiGRU,96.00)

    };
\addlegendentry{CodeT5$^+$}
    
\addplot[mark=triangle*, magenta, solid, every mark/.append style={solid, fill=magenta}]
    coordinates {
    (Base,94.78)
(LSTM,94.24)
(BiLSTM,94.01)
(GRU,94.40)
(BiGRU,93.94)

    };
\addlegendentry{DeepSeek-Coder}

\end{axis}

==> accuracy_scores_SearchSortAlg.tex <==
\begin{axis}[
    ybar=.08cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=5.9cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.2,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.22)},
    anchor=north, legend columns=-2},
    ymin=90, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    symbolic x coords={RoBERTa, CodeBERT, CodeT5, CodeT5$^+$},
    xtick=data,
    %nodes near coords,
    ytick={10, 20, 30, 40, 50, 60, 70, 80, 90, 91, 92, 93, 94, 95, 96, 97, 98, 99, 100},
    %x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=4pt,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
\addplot [draw=Sepia, semithick, pattern=grid, pattern color = Sepia] coordinates {(RoBERTa,95.69) (CodeBERT,96.17) (CodeT5, 96.72) (CodeT5$^+$, 95.97)};  % Macro F1-Score for 0.001

\addplot  [draw=red, semithick, pattern=bricks,  pattern color = red]  coordinates {(RoBERTa,96.26) (CodeBERT,96.33) (CodeT5, 96.68) (CodeT5$^+$, 96.37)};  % Macro F1-Score for 0.005

\addplot  [draw=OliveGreen, semithick, pattern=crosshatch dots,  pattern color = OliveGreen] coordinates {(RoBERTa,96.00) (CodeBERT,96.10) (CodeT5, 96.31) (CodeT5$^+$, 96.42)}; % Macro F1-Score for 0.01

\addplot [draw=blue, semithick, pattern=north west lines,  pattern color = blue] coordinates {(RoBERTa,96.00) (CodeBERT,96.30) (CodeT5,96.32) (CodeT5$^+$, 96.34)}; % Macro F1-Score for 0.01

%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

\legend{LSTM, BiLSTM, GRU, BiGRU}
\end{axis}
 




==> accuracy_scores_SearchSortAlg_curve.tex <==

\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    %xlabel={$minSup$},
    ylabel={$\mathbf{A}$ (\%)},
    ylabel near ticks, ylabel shift={-5pt},
    width=\linewidth,
    width=5.9cm,
    height=4cm,
    grid,
    grid style={gray!50},
    grid=both,
    ymax=97.5,
    ymin=94,
    %xmin=0, xmax=13,
    %ymin=20, ymax=75,
    % xtick={0,20,40,60,80,100},
    ytick={90,91,92,93,94,95,96,97,98},
    %legend style={at={(axis cs:10,60)},anchor=south east},
    symbolic x coords={Base, LSTM, BiLSTM, GRU, BiGRU},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    ymajorgrids=true,
    grid style=solid,
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    %legend style={at={(0.5,-0.20)},
    legend style={at={(0.9,1.05)}, draw=none, anchor=south, legend columns=5},
    %legend style={draw=none},
    %anchor=north, legend columns=3},
]

%\addplot [mark=*, red, dashed] table[x=N,y=No_Sym] {data.dat};


\addplot[mark=otimes*, orange, solid, every mark/.append style={solid, fill=orange}]
    coordinates {
(Base,94.55)
(LSTM,95.69)
(BiLSTM,96.26)
(GRU,96)
(BiGRU,96)
    };
    \addlegendentry{RoBERTa}
    
\addplot[mark=square*, blue, solid, every mark/.append style={solid, fill=blue}]
    coordinates {
(Base,94.80)
(LSTM,96.17)
(BiLSTM,96.33)
(GRU,96.10)
(BiGRU,96.30)


    };
\addlegendentry{CodeBERT}

\addplot[mark=diamond*, red, solid, every mark/.append style={solid, fill=red}]
    coordinates {
(Base,94.88)
(LSTM,96.72)
(BiLSTM,96.68)
(GRU,96.31)
(BiGRU,96.32)
    };
\addlegendentry{CodeT5}

\addplot[mark=*, teal, solid, every mark/.append style={solid, fill=teal}]
    coordinates {
(Base,96.43)
(LSTM,95.97)
(BiLSTM,96.37)
(GRU,96.42)
(BiGRU,96.34)

    };
\addlegendentry{CodeT5$^+$}
    
\addplot[mark=triangle*, magenta, solid, every mark/.append style={solid, fill=magenta}]
    coordinates {
(Base,97.23)
(LSTM,96.78)
(BiLSTM,96.71)
(GRU,96.58)
(BiGRU,96.78)

    };
\addlegendentry{DeepSeek-Coder}
\legend{};
\end{axis}

==> accuracy_scores_SearchSortGTAlg.tex <==
\begin{axis}[
    ybar=.08cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=5.9cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.2,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.22)},
    anchor=north, legend columns=-2},
    ymin=90, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    symbolic x coords={RoBERTa, CodeBERT, CodeT5, CodeT5$^+$},
    xtick=data,
    %nodes near coords,
    ytick={10, 20, 30, 40, 50, 60, 70, 80, 90, 91, 92, 93, 94, 95, 96, 97, 98, 99, 100},
    %x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=4pt,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
\addplot [draw=orange, semithick, pattern=grid, pattern color = orange] coordinates {(RoBERTa,95.19) (CodeBERT,96.02) (CodeT5, 96.07) (CodeT5$^+$, 96.08)};  % Macro F1-Score for 0.001

\addplot [draw=teal, semithick, pattern=bricks,  pattern color = teal] coordinates {(RoBERTa,95.36) (CodeBERT,95.75) (CodeT5, 96.07) (CodeT5$^+$, 96.27)};  % Macro F1-Score for 0.005

\addplot [draw=gray, semithick, pattern=crosshatch dots,  pattern color = gray] coordinates {(RoBERTa,95.45) (CodeBERT,96.05) (CodeT5, 95.44) (CodeT5$^+$, 95.92)}; % Macro F1-Score for 0.01

\addplot [draw=blue, semithick, pattern=north west lines,  pattern color = blue] coordinates {(RoBERTa,96.00) (CodeBERT,95.75) (CodeT5,95.06) (CodeT5$^+$, 96.03)}; % Macro F1-Score for 0.01

%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

\legend{LSTM, BiLSTM, GRU, BiGRU}
\end{axis}
 


==> accuracy_scores_SearchSortGTAlg_curve.tex <==

\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    %xlabel={$minSup$},
    ylabel={$\mathbf{A}$ (\%)},
    ylabel near ticks, ylabel shift={-5pt},
    width=\linewidth,
    width=5.9cm,
    height=4cm,
    grid,
    grid style={gray!50},
    grid=both,
    ymax=97,
    ymin=92,
    %xmin=0, xmax=13,
    %ymin=20, ymax=75,
    % xtick={0,20,40,60,80,100},
    ytick={90,91,92,93,94,95,96,97,98},
    %legend style={at={(axis cs:10,60)},anchor=south east},
    symbolic x coords={Base, LSTM, BiLSTM, GRU, BiGRU},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    ymajorgrids=true,
    grid style=solid,
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    legend style={at={(0.5,-0.20)},
    legend style={draw=none},
    anchor=north, legend columns=3},
]

%\addplot [mark=*, red, dashed] table[x=N,y=No_Sym] {data.dat};


\addplot[mark=otimes*, orange, solid, every mark/.append style={solid, fill=orange}]
    coordinates {
    (Base,92.92)
(LSTM,95.19)
(BiLSTM,95.36)
(GRU,95.45)
(BiGRU,96)
    };
    \addlegendentry{RoBERTa}
    
\addplot[mark=square*, blue, solid, every mark/.append style={solid, fill=blue}]
    coordinates {
    (Base,93.36)
(LSTM,96.02)
(BiLSTM,95.75)
(GRU,96.05)
(BiGRU,95.75)


    };
\addlegendentry{CodeBERT}

\addplot[mark=diamond*, red, solid, every mark/.append style={solid, fill=red}]
    coordinates {
(Base,96.15)
(LSTM,96.07)
(BiLSTM,96.07)
(GRU,95.44)
(BiGRU,95.06)
    };
\addlegendentry{CodeT5}

\addplot[mark=*, teal, solid, every mark/.append style={solid, fill=teal}]
    coordinates {
    (Base,96.28)
(LSTM,96.08)
(BiLSTM,96.27)
(GRU,95.92)
(BiGRU,96.03)

    };
\addlegendentry{CodeT5$^+$}
    
\addplot[mark=triangle*, magenta, solid, every mark/.append style={solid, fill=magenta}]
    coordinates {
    (Base,94.87)
(LSTM,92.86)
(BiLSTM,93.03)
(GRU,93.47)
(BiGRU,92.97)

    };
\addlegendentry{DeepSeek-Coder}
\legend{};
\end{axis}

==> augmented_roberta_bilstm.tex <==
\begin{axis}[
    ybar=.2cm,
    every node near coord/.append style={font=\scriptsize},
    legend style={font=\scriptsize},
    tick label style={font=\scriptsize},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    width=\linewidth,
    %width=7.5cm,
    height=5.2cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.50,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.22)},
    anchor=north, legend columns=-1},
    ymin=50, 
    ylabel={Score (\%)},
    %xlabel={Datasets},
    symbolic x coords={Pre-Augmentation, Post-Augmentation},
    xtick=data,
    nodes near coords,
    ytick={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    %x tick label style={rotate=25,anchor=east},
    grid=both,
    %nodes near coords,
    nodes near coords align={vertical},
    bar width=14pt,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]

\addplot [draw=Green, color=Green, semithick, pattern=north east lines, pattern color = Green] coordinates {(Pre-Augmentation,80.94) (Post-Augmentation,95.91) };  % Macro F1-Score for 0.001

\addplot [draw=Blue, color=Blue, semithick, pattern=crosshatch dots, pattern color = Blue] coordinates {(Pre-Augmentation,80.74) (Post-Augmentation,95.77) };  % Macro F1-Score for 0.001


\addplot [draw=Red, color=Red, semithick, pattern=horizontal lines, pattern color = Red] coordinates {(Pre-Augmentation,80.73) (Post-Augmentation,95.74) };  % Macro F1-Score for 0.001

\addplot [draw=teal, color=teal, semithick, pattern=grid,  pattern color = teal] coordinates {(Pre-Augmentation,80.74) (Post-Augmentation,95.77)};  % Macro F1-Score for 0.005

%\addplot [draw=magenta, semithick, pattern=crosshatch dots,  pattern color = magenta] coordinates {(IMDb,91.24) (Twitter US Airline,79.37) (Sentiment140,81.81)}; % Macro F1-Score for 0.01

%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

\legend{$\mathbf{P}_\psi$, $\mathbf{R}_\psi$, $\mathbf{F1}_\psi$, $\mathbf{A}$}
\end{axis}
 


==> biomedical_accuracy.tex <==
\begin{axis}[
    ybar=.05cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    width=\textwidth,
    %width=8cm,
    height=6.5cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.08,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=86.5, 
    ylabel={$\mathbf{A}$  (\%)},
    %xlabel={Datasets},
    %symbolic x coords={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
    %xtick=data,
    xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20},
    %nodes near coords,
    ytick={85, 86, 87, 88, 89, 90,91,92,93,94},
    xticklabels={RoBERTa-base, -GRU, -LSTM, -BiLSTM, -BiGRU, BioLinkBERT-base, -GRU, -LSTM, -BiLSTM, -BiGRU, GPT2, -GRU, -LSTM, -BiLSTM, -BiGRU, DeepSeek-R1, -GRU, -LSTM, -BiLSTM, -BiGRU},
    x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=10pt,
    bar shift=0,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
%\addplot [draw=black, semithick, color=red, preaction={fill, red}, pattern=crosshatch dots, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.31) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.35)};  %  F1w Scores 

%\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)};  % A Scores 





\addplot [draw=black, color=OrangeRed, preaction={fill, OrangeRed}, semithick, pattern color = white] coordinates {(1,88.15)}; % RoBERTa-base

\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern color = white]coordinates {(2,88.40)}; % RoBERTa-GRU

\addplot[draw=black, color=ForestGreen, preaction={fill, ForestGreen}, semithick,  pattern color = white]coordinates {(3,88.75)}; % RoBERTa-LSTM

\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern color = white] coordinates {(4,88.31)}; % RoBERTa-BiLSTM

\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern color = white] coordinates {(5,88.35)}; % RoBERTa-BiGRU


\addplot [draw=black, color=OrangeRed, preaction={fill, OrangeRed}, semithick, pattern=grid, pattern color = white] coordinates {(6,88.26)}; % BioLinkBERT-base

\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern=grid, pattern color = white]coordinates {(7,88.40)}; % BioLinkBERT-GRU

\addplot[draw=black, color=ForestGreen, preaction={fill, ForestGreen}, semithick, pattern=grid, pattern color = white]coordinates {(8,88.33)}; % BioLinkBERT-LSTM

\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(9,88.37)}; % BioLinkBERT-BiLSTM

\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white] coordinates {(10,88.36)}; % BioLinkBERT-BiGRU





\addplot [draw=black, color=OrangeRed, preaction={fill, OrangeRed}, semithick, pattern color = white] coordinates {(11,93.52)}; % GPT2

\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern color = white]coordinates {(12,93.41)}; % GPT2-GRU

\addplot[draw=black, color=ForestGreen, preaction={fill, ForestGreen}, semithick,  pattern color = white]coordinates {(13,93.62)}; % GPT2-LSTM

\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern color = white] coordinates {(14,92.03)}; % GPT2-BiLSTM

\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern color = white] coordinates {(15,93.62)}; % GPT2-BiGRU


\addplot [draw=black, color=OrangeRed, preaction={fill, OrangeRed}, semithick, pattern=grid, pattern color = white] coordinates {(16,93.20)}; % DS-R1

\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern=grid, pattern color = white]coordinates {(17,93.41)}; % DS-R1-GRU

\addplot[draw=black, color=ForestGreen, preaction={fill, ForestGreen}, semithick, pattern=grid, pattern color = white]coordinates {(18,93.73)}; % DS-R1-LSTM

\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(19,92.88)}; % DS-R1-BiLSTM

\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white] coordinates {(20,92.45)}; % DS-R1-BiGRU



%(BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)







%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

%\legend{$\mathbf{F1}_w$ Score, $\mathbf{A}$ Score}
\end{axis}
 


==> biomedical_accuracy_best_results.tex <==
\begin{axis}[
    ybar=.05cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=8cm,
    height=5cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.08,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=86.5, 
    ylabel={$\mathbf{A}$  (\%)},
    %xlabel={Datasets},
    %symbolic x coords={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
    %xtick=data,
    xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20},
    %nodes near coords,
    ytick={85, 86, 87, 88, 89, 90,91,92,93,94},
    xticklabels={RoBERTa-base,  -LSTM, BioLinkBERT-base, -GRU,  GPT2,  -LSTM, DeepSeek-R1,  -LSTM},
    x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=10pt,
    bar shift=0,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
%\addplot [draw=black, semithick, color=red, preaction={fill, red}, pattern=crosshatch dots, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.31) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.35)};  %  F1w Scores 

%\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)};  % A Scores 





\addplot [draw=black, color=OrangeRed, preaction={fill, OrangeRed}, semithick, pattern color = white] coordinates {(1,88.15)}; % RoBERTa-base

%\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern color = white]coordinates {(2,88.40)}; % RoBERTa-GRU

\addplot[draw=black, color=ForestGreen, preaction={fill, ForestGreen}, semithick,  pattern color = white]coordinates {(2,88.75)}; % RoBERTa-LSTM

%\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern color = white] coordinates {(4,88.31)}; % RoBERTa-BiLSTM

%\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern color = white] coordinates {(5,88.35)}; % RoBERTa-BiGRU


\addplot [draw=black, color=OrangeRed, preaction={fill, OrangeRed}, semithick, pattern=grid, pattern color = white] coordinates {(3,88.26)}; % BioLinkBERT-base

\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern=grid, pattern color = white]coordinates {(4,88.40)}; % BioLinkBERT-GRU

%\addplot[draw=black, color=ForestGreen, preaction={fill, ForestGreen}, semithick, pattern=grid, pattern color = white]coordinates {(8,88.33)}; % BioLinkBERT-LSTM

%\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(9,88.37)}; % BioLinkBERT-BiLSTM

%\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white] coordinates {(10,88.36)}; % BioLinkBERT-BiGRU





\addplot [draw=black, color=Blue, preaction={fill, Blue}, semithick, pattern color = white] coordinates {(5,93.52)}; % GPT2

%\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern color = white]coordinates {(12,93.41)}; % GPT2-GRU

\addplot[draw=black, color=Red, preaction={fill, Red}, semithick,  pattern color = white]coordinates {(6,93.62)}; % GPT2-LSTM

%\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern color = white] coordinates {(14,92.03)}; % GPT2-BiLSTM

%\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern color = white] coordinates {(7,93.62)}; % GPT2-BiGRU


\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(7,93.20)}; % DS-R1

%\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern=grid, pattern color = white]coordinates {(17,93.41)}; % DS-R1-GRU

\addplot[draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white]coordinates {(8,93.73)}; % DS-R1-LSTM

%\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(19,92.88)}; % DS-R1-BiLSTM

%\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white] coordinates {(20,92.45)}; % DS-R1-BiGRU



%(BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)







%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

%\legend{$\mathbf{F1}_w$ Score, $\mathbf{A}$ Score}
\end{axis}
 


==> codebert-bilstm-defect-detection.tex <==
\begin{axis}[
    ybar=.12cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=8cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.25,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.25)},
    anchor=north, legend columns=4},
    ymin=30, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    symbolic x coords={AdamW, NAdam, RMSProp},
    xtick=data,
    %nodes near coords,
    ytick={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    %x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=9pt,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
\addplot [draw=black, semithick, pattern=north west lines, pattern color = black] coordinates {(AdamW,54.06) (NAdam,54.06) (RMSProp, 54.06)};  % Macro F1-Score for 0.001

\addplot [draw=black, semithick, pattern=horizontal lines,  pattern color = black] coordinates {(AdamW,64.14) (NAdam,64.62) (RMSProp, 63.25)};  % Macro F1-Score for 0.005

\addplot [draw=black, semithick, pattern=dots,  pattern color = black] coordinates {(AdamW,64.19) (NAdam,64.48) (RMSProp, 63.91)}; % Macro F1-Score for 0.01

\addplot [draw=black, semithick, pattern=bricks,  pattern color = black] coordinates {(AdamW,61.87) (NAdam,61.81) (RMSProp,61.36)}; % Macro F1-Score for 0.01

%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

\legend{$1e^{-4}$, $2e^{-5}$, $1e^{-5}$, $1e^{-6}$}
\end{axis}
 


==> codet5_lstm_accu_performance_with_lr_nadam.tex <==

\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    %xlabel={$minSup$},
    ylabel={$\mathbf{A}$ (\%)},
    ylabel near ticks, ylabel shift={-5pt},
    %width=\textwidth,
    width=4.7cm,
    height=4cm,
    grid,
    grid style={gray!50},
    grid=both,
    ymin=55,
    ymax=70,
    %xmin=0, xmax=13,
    %ymin=20, ymax=75,
    % xtick={0,20,40,60,80,100},
    ytick={50, 55, 60, 65, 70},
    %legend style={at={(axis cs:10,60)},anchor=south east},
    symbolic x coords={$l=1e^{-4}$, $l=2e^{-5}$, $l=1e^{-5}$, $l=1e^{-6}$},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    ymajorgrids=true,
    grid style=solid,
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    legend style={at={(0.35,0.65)},
    legend style={draw=none},
    anchor=north, legend columns=1},
]

%\addplot [mark=*, red, dashed] table[x=N,y=No_Sym] {data.dat};


\addplot[mark=otimes*, black, dashed, every mark/.append style={solid, fill=black}]
    coordinates {
($l=1e^{-4}$,66.22)
($l=2e^{-5}$,66.58)
($l=1e^{-5}$,65.87)
($l=1e^{-6}$,56.23)
    };
    \addlegendentry{LSTM}
    
\addplot[mark=diamond*, blue, dashed, every mark/.append style={solid, fill=blue}]
    coordinates {
($l=1e^{-4}$,65.32)
($l=2e^{-5}$,65.78)
($l=1e^{-5}$,66.64)
($l=1e^{-6}$,57.61)


    };
    \addlegendentry{BiLSTM}

\addplot[mark=square*, red, dashed, every mark/.append style={solid, fill=red}]
    coordinates {
($l=1e^{-4}$,65.58)
($l=2e^{-5}$,65.02)
($l=1e^{-5}$,65.61)
($l=1e^{-6}$,56.70)

    };
    \addlegendentry{GRU}
    

\addplot[mark=oplus*, teal, dashed, every mark/.append style={solid, fill=teal}]
    coordinates {
($l=1e^{-4}$,66.36)
($l=2e^{-5}$,65.75)
($l=1e^{-5}$,65.62)
($l=1e^{-6}$,57.06)

    };
    \addlegendentry{BiGRU}


\end{axis}

==> codet5_lstm_accuracy_performance_with_lr.tex <==

\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    %xlabel={$minSup$},
    ylabel={$\mathbf{A}$ (\%)},
    ylabel near ticks, ylabel shift={-5pt},
    %width=\textwidth,
    width=4.7cm,
    height=4cm,
    grid,
    grid style={gray!50},
    grid=both,
    ymin=55,
    ymax=70,
    %xmin=0, xmax=13,
    %ymin=20, ymax=75,
    % xtick={0,20,40,60,80,100},
    ytick={50, 55, 60, 65, 70,75},
    %legend style={at={(axis cs:10,60)},anchor=south east},
    symbolic x coords={$l=1e^{-4}$, $l=2e^{-5}$, $l=1e^{-5}$, $l=1e^{-6}$},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    ymajorgrids=true,
    grid style=solid,
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    %legend style={at={(0.5,-0.42)},
    legend style={at={(0.35,0.65)},
    legend style={draw=none},
    anchor=north, legend columns=1},
]

%\addplot [mark=*, red, dashed] table[x=N,y=No_Sym] {data.dat};


\addplot[mark=otimes*, black, dashed, every mark/.append style={solid, fill=black}]
    coordinates {
($l=1e^{-4}$,66.40)
($l=2e^{-5}$,66.51)
($l=1e^{-5}$,65.50)
($l=1e^{-6}$,56.60)
    };
    \addlegendentry{LSTM}
    
\addplot[mark=diamond*, blue, dashed, every mark/.append style={solid, fill=blue}]
    coordinates {
($l=1e^{-4}$,65.17)
($l=2e^{-5}$,66.03)
($l=1e^{-5}$,65.91)
($l=1e^{-6}$,56.98)


    };
    \addlegendentry{BiLSTM}

\addplot[mark=square*, red, dashed, every mark/.append style={solid, fill=red}]
    coordinates {
($l=1e^{-4}$,66.76)
($l=2e^{-5}$,66.14)
($l=1e^{-5}$,63.59)
($l=1e^{-6}$,56.41)

    };
    \addlegendentry{GRU}
    

\addplot[mark=oplus*, teal, dashed, every mark/.append style={solid, fill=teal}]
    coordinates {
($l=1e^{-4}$,65.86)
($l=2e^{-5}$,65.63)
($l=1e^{-5}$,66.01)
($l=1e^{-6}$,56.48)

    };
    \addlegendentry{BiGRU}


\end{axis}

==> energy_mistral_squad.tex <==

\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    %xlabel={$minSup$},
    ylabel={Total Energy (kWh)},
    xlabel={Token Generation},
    ylabel near ticks, ylabel shift={-5pt},
    xlabel shift={-8pt},
    width=\linewidth,
    width=5.1cm,
    height=4cm,
    grid,
    grid style={gray!50},
    grid=both,
    %ymode=log,                         % <-- use log scale here
    %log basis y={10},                 % base-10 log scale
    %ymin=100, ymax=2000,             % adjust range for log scale
    %ymax=132,
    %xmin=0, xmax=13,
    %ymin=20, ymax=75,
    % xtick={0,20,40,60,80,100},
    ytick={0,0.5,1.0,1.5,2.0,2.5,3.0,3.5,4.0,4.5,5.0,5.5,6.0,6.5,7.0},
    %legend style={at={(axis cs:10,60)},anchor=south east},
    symbolic x coords={512,1024, 2048,3000},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    ymajorgrids=true,
    grid style=solid,
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    legend style={at={(0.5,-0.10)},
    legend style={draw=none},
    anchor=north, legend columns=3},
]

%\addplot [mark=*, red, dashed] table[x=N,y=No_Sym] {data.dat};


\addplot[mark=otimes*, black, solid, every mark/.append style={solid, fill=black}]
    coordinates {
(512,1.1310)
(1024,2.330)
(2048,4.334)
(3000,6.8001)
    };
    \addlegendentry{Base(1k)}
    
\addplot[mark=otimes*, black, dashdotted, every mark/.append style={solid, fill=black}]
    coordinates {
(512,1.0664)
(1024,2.111)
(2048,3.658)
(3000,5.3483)
    };
    \addlegendentry{CMC(1k)}
    


\addplot[mark=square*, Green, solid, every mark/.append style={solid, fill=Green}]
    coordinates {
(512,0.4993)
(1024,1.1956)
(2048,2.6209)
(3000,4.1743)
    };
\addlegendentry{Base (512)}

\addplot[mark=square*, Green, dashdotted, every mark/.append style={solid, fill=Green}]
    coordinates {
(512,0.4756)
(1024,1.1411)
(2048,2.1367)
(3000,3.2237)

    };
\addlegendentry{CMC (512)}


\addplot[mark=diamond*, magenta, solid, every mark/.append style={solid, fill=magenta}]
    coordinates {
(512,0.2478)
(1024,0.5213)
(2048,1.1089)
(3000,2.0895)
    };
\addlegendentry{Base (256)}

\addplot[mark=diamond*, magenta, dashdotted, every mark/.append style={solid, fill=magenta}]
    coordinates {
(512,0.2357)
(1024,0.4749)
(2048,0.9373)
(3000,1.6066)
    };
\addlegendentry{CMC (256)}





\end{axis}

==> imdb_bar.tex <==
 \begin{axis}[
        /pgf/number format/1000 sep={},
         width=6.3cm,
         height=4.5cm,
        at={(0.758in,0.981in)},
        scale only axis,
        clip=false,
        separate axis lines,
        axis on top,
        xmin=0,
        xmax=5,
        xtick={1,2,3,4,5,6,7,8,9,10},
        x tick style={draw=none},
    xticklabels={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
        ytick={0,500,1000, 2000},
        ymin=0,
        %ymax=2000,
        ylabel={YYY},
        every axis plot/.append style={
          ybar,
          bar width=.2,
          bar shift=0pt,
          fill
        }
      ]
\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(1,91.24)};

\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(2,91.24)};
\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(3,91.24)};
\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(4,91.24)};
\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(5,91.24)};

\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(6,91.32)};

\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(7,91.68)};

\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(8,91.80)};
\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(9,92.36)};

\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(10,91.24)};
    \end{axis}

==> performance-comparison-imbd.tex <==
\begin{axis}[
    ybar=.05cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=5.7cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.08,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=90, 
    ylabel={$\mathbf{A}$  (\%)},
    %xlabel={Datasets},
    %symbolic x coords={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
    %xtick=data,
    xtick={1,2,3,4,5,6,7,8},
    %nodes near coords,
    ytick={90, 90.50, 91, 91.50, 92, 92.50},
    xticklabels={BERT-base, -LSTM, -GRU, -BiLSTM, RoBERTa-base, -GRU, -LSTM, -BiLSTM},
    x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=6pt,
    bar shift=0,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
%\addplot [draw=black, semithick, color=red, preaction={fill, red}, pattern=crosshatch dots, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.31) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.35)};  %  F1w Scores 

%\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)};  % A Scores 



\addplot [draw=blue, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white]  coordinates {(1,90.96)}; % BERT-base

\addplot  [draw=blue, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white]   coordinates {(2,91.32)}; % BERT-LSTM

\addplot  [draw=blue, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white]  coordinates {(3,91.12)}; % BERT-GRU

\addplot [draw=blue, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white]   coordinates {(4,91.24)}; % BERT-BiLSTM

\addplot [draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white] coordinates {(5,91.32)}; % RoBERTa-base

\addplot [draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white]coordinates {(6,92.60)}; % RoBERTa-GRU

\addplot[draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white]coordinates {(7,92.04)}; % RoBERTa-LSTM

\addplot [draw=black, color=red, preaction={fill, red}, semithick, pattern=grid, pattern color = white] coordinates {(8,92.36)}; % RoBERTa-BiLSTM



%(BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)







%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

%\legend{$\mathbf{F1}_w$ Score, $\mathbf{A}$ Score}
\end{axis}
 


==> performance-comparison-sentiment140.tex <==
\begin{axis}[
    ybar=.05cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=5.7cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.08,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=81, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    %symbolic x coords={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
    %xtick=data,
    xtick={1,2,3,4,5,6,7,8},
    %nodes near coords,
    ytick={81, 81.5, 82, 82.5},
    xticklabels={BERT-base, -LSTM, -GRU, -BiLSTM, RoBERTa-base, -GRU, -LSTM, -BiLSTM},
    x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=6pt,
    bar shift=0,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
%\addplot [draw=black, semithick, color=red, preaction={fill, red}, pattern=crosshatch dots, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.31) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.35)};  %  F1w Scores 

%\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)};  % A Scores 



\addplot  [draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white] coordinates {(1,81.35)}; % BERT-base

\addplot   [draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white]  coordinates {(2,81.75)}; % BERT-LSTM

\addplot  [draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white]   coordinates {(3,81.83)}; % BERT-GRU

\addplot  [draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white]  coordinates {(4,81.81)}; % BERT-BiLSTM

\addplot [draw=black, color=Purple, preaction={fill, Purple}, semithick, pattern=grid, pattern color = white] coordinates {(5,82.17)}; % RoBERTa-base

\addplot [draw=black, color=Purple, preaction={fill, Purple}, semithick, pattern=grid, pattern color = white] coordinates {(6,82.32)}; % RoBERTa-GRU

\addplot[draw=black, color=Purple, preaction={fill, Purple}, semithick, pattern=grid, pattern color = white] coordinates {(7,82.29)}; % RoBERTa-LSTM

\addplot [draw=black, color=Purple, preaction={fill, Purple}, semithick, pattern=grid, pattern color = white] coordinates {(8,82.25)}; % RoBERTa-BiLSTM



%(BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)







%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

%\legend{$\mathbf{F1}_w$ Score, $\mathbf{A}$ Score}
\end{axis}
 


==> performance-comparison-twitter.tex <==
\begin{axis}[
    ybar=.05cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=5.7cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.08,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=74, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    %symbolic x coords={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
    %xtick=data,
    xtick={1,2,3,4,5,6,7,8},
    %nodes near coords,
    ytick={71, 72, 73, 74, 75, 76, 77, 78, 79, 80, 81},
    xticklabels={BERT-base, -LSTM, -GRU, -BiLSTM, RoBERTa-base, -GRU, -LSTM, -BiLSTM},
    x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=6pt,
    bar shift=0,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
%\addplot [draw=black, semithick, color=red, preaction={fill, red}, pattern=crosshatch dots, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.31) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.35)};  %  F1w Scores 

%\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)};  % A Scores 



\addplot [draw=blue, color=teal, preaction={fill, teal}, semithick, pattern=grid, pattern color = white]  coordinates {(1,75.27)}; % BERT-base

\addplot [draw=blue, color=teal, preaction={fill, teal}, semithick, pattern=grid, pattern color = white]   coordinates {(2,78.83)}; % BERT-LSTM

\addplot [draw=blue, color=teal, preaction={fill, teal}, semithick, pattern=grid, pattern color = white]   coordinates {(3,78.83)}; % BERT-GRU

\addplot [draw=blue, color=teal, preaction={fill, teal}, semithick, pattern=grid, pattern color = white]   coordinates {(4,79.37)}; % BERT-BiLSTM

\addplot [draw=black, color=Magenta, preaction={fill, Magenta}, semithick, pattern=grid, pattern color = white] coordinates {(5,79.78)}; % RoBERTa-base

\addplot [draw=black, color=Magenta, preaction={fill, Magenta}, semithick, pattern=grid, pattern color = white] coordinates {(6,79.92)}; % RoBERTa-GRU

\addplot [draw=black, color=Magenta, preaction={fill, Magenta}, semithick, pattern=grid, pattern color = white] coordinates {(7,80.33)}; % RoBERTa-LSTM

\addplot [draw=black, color=Magenta, preaction={fill, Magenta}, semithick, pattern=grid, pattern color = white] coordinates {(8,80.74)}; % RoBERTa-BiLSTM



%(BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)







%\addplot [draw=black, semithick, pattern=grid, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

%\legend{$\mathbf{F1}_w$ Score, $\mathbf{A}$ Score}
\end{axis}
 


==> roberta-bilstm-twitter.tex <==
\begin{axis}[
    ybar=.1cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=4.5cm,
    height=3.5cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.25,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=30, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    symbolic x coords={$h=128$, $h=256$, $h=512$},
    xtick=data,
    %nodes near coords,
    ytick={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    %x tick label style={rotate=25,anchor=east},
    grid=both,
    %nodes near coords,
    nodes near coords align={vertical},
    bar width=5pt,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
\addplot [draw=olive, semithick, pattern=crosshatch dots, pattern color = olive] coordinates {($h=128$,65.44) ($h=256$,68.31) ($h=512$,59.84)};  % Macro F1-Score for 0.001

\addplot [draw=blue, semithick, pattern=north west lines,  pattern color = blue] coordinates {($h=128$,78.01) ($h=256$,80.74) ($h=512$,80.33)};  % Macro F1-Score for 0.005

\addplot [draw=orange, semithick, pattern=horizontal lines,  pattern color = orange] coordinates {($h=128$,79.10) ($h=256$,78.69) ($h=512$,78.42)}; % Macro F1-Score for 0.01

%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

\legend{$1e^{-4}$, $1e^{-5}$, $1e^{-6}$}
\end{axis}
 


==> roberta-gru-sentiment140.tex <==
\begin{axis}[
    ybar=.1cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=4.5cm,
    height=3.5cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.25,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    ymin=30, 
    ylabel={$\mathbf{A}$ (\%)},
    %xlabel={Datasets},
    symbolic x coords={$h=128$, $h=256$, $h=512$},
    xtick=data,
    %nodes near coords,
    ytick={10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    %x tick label style={rotate=25,anchor=east},
    grid=both,
    %nodes near coords,
    nodes near coords align={vertical},
    bar width=6pt,
    %ymajorgrids=true,
    label style={font=\footnotesize},
    ]
\addplot [draw=red, semithick, pattern=north west lines, pattern color = red] coordinates {($h=128$,49.83) ($h=256$,49.83) ($h=512$,49.83)};  % Macro F1-Score for 0.001

\addplot [draw=blue, semithick, pattern=grid,  pattern color = blue] coordinates {($h=128$,82.25) ($h=256$,82.32) ($h=512$,82.21)};  % Macro F1-Score for 0.005

\addplot [draw=teal, semithick, pattern=crosshatch dots,  pattern color = teal] coordinates {($h=128$,81.62) ($h=256$,81.62) ($h=512$,81.63)}; % Macro F1-Score for 0.01

%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

\legend{$1e^{-4}$, $1e^{-5}$, $1e^{-6}$}
\end{axis}
 


==> test_curve.tex <==
\begin{axis}[
    ylabel={$\mathbf{A}$ (\%)},
    ylabel near ticks, ylabel shift={-5pt},
    width=5.9cm,
    height=4cm,
    grid=both,
    ymin=93,
    ytick={90,91,92,93,94,95,96,97},
    symbolic x coords={LSTM, BiLSTM, GRU, BiGRU},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    tick label style={font=\tiny},
]

\addplot[mark=otimes*, orange, solid, every mark/.append style={solid, fill=orange}]
    coordinates {(LSTM,93.44)(BiLSTM,93.55)(GRU,93.44)(BiGRU,93.59)}
    node[pos=0.5, below] {\tiny RoBERTa};

\addplot[mark=square*, blue, solid, every mark/.append style={solid, fill=blue}]
    coordinates {(LSTM,93.59)(BiLSTM,94.01)(GRU,93.82)(BiGRU,93.97)}
    node[pos=0.25, above] {\tiny CodeBERT};

\addplot[mark=diamond*, red, solid, every mark/.append style={solid, fill=red}]
    coordinates {(LSTM,94.40)(BiLSTM,95.12)(GRU,94.17)(BiGRU,94.86)}
    node[pos=0.25, above] {\tiny CodeT5};

\addplot[mark=*, teal, solid, every mark/.append style={solid, fill=teal}]
    coordinates {(LSTM,95.00)(BiLSTM,96.00)(GRU,96.00)(BiGRU,96.00)}
    node[pos=0.25, above] {\tiny CodeT5$^+$};

\addplot[mark=triangle*, magenta, solid, every mark/.append style={solid, fill=magenta}]
    coordinates {(LSTM,94.24)(BiLSTM,94.01)(GRU,94.40)(BiGRU,93.94)}
    node[pos=0.75, above] {\tiny DeepSeek-Coder};

\end{axis}


==> time_curve.tex <==

\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    %xlabel={$minSup$},
    ylabel={Trainig Time (s)},
    ylabel near ticks, ylabel shift={-5pt},
    width=\linewidth,
    width=4.6cm,
    height=4cm,
    grid,
    grid style={gray!50},
    grid=both,
    %ymin=1500,
    %xmin=0, xmax=13,
    %ymin=20, ymax=75,
    % xtick={0,20,40,60,80,100},
    %ytick={60, 65, 70, 75, 80, 85, 90, 95, 100},
    %legend style={at={(axis cs:10,60)},anchor=south east},
    symbolic x coords={RoBERTa, CodeBERT, CodeT5, CodeT5$^+$},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    ymajorgrids=true,
    grid style=solid,
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    legend style={at={(0.5,-0.22)},
    legend style={draw=none},
    anchor=north, legend columns=2},
]

%\addplot [mark=*, red, dashed] table[x=N,y=No_Sym] {data.dat};


\addplot[mark=otimes*, orange, dashdotted, every mark/.append style={solid, fill=orange}]
    coordinates {
(RoBERTa,2767)
(CodeBERT,2763)
(CodeT5,3133)
(CodeT5$^+$,3140)

    };
    \addlegendentry{Base}
    
\addplot[mark=square*, blue, dashdotted, every mark/.append style={solid, fill=blue}]
    coordinates {
(RoBERTa,2913)
(CodeBERT,3043)
(CodeT5,3169)
(CodeT5$^+$,3492)


    };
\addlegendentry{LSTM}

\addplot[mark=diamond*, red, dashdotted, every mark/.append style={solid, fill=red}]
    coordinates {
(RoBERTa,3190)
(CodeBERT,3083)
(CodeT5,3271)
(CodeT5$^+$,3426)
    };
\addlegendentry{BiLSTM}

\addplot[mark=*, teal, dashdotted, every mark/.append style={solid, fill=teal}]
    coordinates {
(RoBERTa,3032)
(CodeBERT,3083)
(CodeT5,3445)
(CodeT5$^+$,3409)

    };
\addlegendentry{GRU}
    
\addplot[mark=triangle*, magenta, dashdotted, every mark/.append style={solid, fill=magenta}]
    coordinates {
(RoBERTa,3153)
(CodeBERT,3160)
(CodeT5,3520)
(CodeT5$^+$,3384)

    };
\addlegendentry{BiGRU}

\end{axis}

==> trainable_param.tex <==
\begin{axis}[
    ybar=.05cm,
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    ylabel near ticks, ylabel shift={-6pt},
    %xlabel shift={-10pt},
    %width=\textwidth,
    width=4.6cm,
    height=4cm,
    every node near coord/.append style={
                        anchor=west,
                        rotate=75
                },
    enlargelimits=.08,
    enlarge y limits={0.1,upper},
    legend style={at={(0.5,-0.32)},
    anchor=north, legend columns=-1},
    %ymin=86.5, 
    ylabel={Trainable Params. (B)},
    %xlabel={Datasets},
    %symbolic x coords={BERT-base, BERT-LSTM, BERT-GRU, BERT-BiLSTM, BERT-BiGRU, RoBERTa-base, RoBERTa-GRU, RoBERTa-LSTM, RoBERTa-BiLSTM, RoBERTa-BiGRU},
    %xtick=data,
    xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19,20},
    %nodes near coords,
    %ytick={0.06, 0.08, 0.10, 0.12, 0.14, 0.16, 1.0, 1.5},
    xticklabels={RoBERTa,  CodeBERT, BioLinkBERT, DeepSeek-R1, DeepSeek-Coder, GPT2, CodeT5, CodeT5P},
    x tick label style={rotate=25,anchor=east},
    grid=both,
    nodes near coords,
    nodes near coords align={vertical},
    bar width=6pt,
    bar shift=0,
    %ymajorgrids=true,
    label style={font=\tiny},
    ]
%\addplot [draw=black, semithick, color=red, preaction={fill, red}, pattern=crosshatch dots, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.31) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.35)};  %  F1w Scores 

%\addplot [draw=black, semithick, pattern=grid, preaction={fill, red}, pattern color = black] coordinates {(BERT-base,91.24) (BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)};  % A Scores 





\addplot [draw=black, color=OrangeRed, preaction={fill, OrangeRed}, semithick, pattern color = white] coordinates {(1,0.13)}; % RoBERTa

%\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern color = white]coordinates {(2,88.40)}; % RoBERTa-GRU

\addplot[draw=black, color=ForestGreen, preaction={fill, ForestGreen}, semithick,  pattern color = white]coordinates {(2,0.13)}; % CodeBERT

%\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern color = white] coordinates {(4,88.31)}; % RoBERTa-BiLSTM

%\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern color = white] coordinates {(5,88.35)}; % RoBERTa-BiGRU


\addplot [draw=black, color=OrangeRed, preaction={fill, OrangeRed}, semithick, pattern=grid, pattern color = white] coordinates {(3,0.11)}; % BioLinkBERT-base

\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern=grid, pattern color = white]coordinates {(4,1.55)}; % DeepSeek-R1

%\addplot[draw=black, color=ForestGreen, preaction={fill, ForestGreen}, semithick, pattern=grid, pattern color = white]coordinates {(8,88.33)}; % BioLinkBERT-LSTM

%\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(9,88.37)}; % BioLinkBERT-BiLSTM

%\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white] coordinates {(10,88.36)}; % BioLinkBERT-BiGRU





\addplot [draw=black, color=Blue, preaction={fill, Blue}, semithick, pattern color = white] coordinates {(5,1.282)}; %DeepSeek-Coder

%\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern color = white]coordinates {(12,93.41)}; % GPT2-GRU

\addplot[draw=black, color=Red, preaction={fill, Red}, semithick,  pattern color = white]coordinates {(6,0.12)}; % GPT2

%\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern color = white] coordinates {(14,92.03)}; % GPT2-BiLSTM

%\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern color = white] coordinates {(7,93.62)}; % GPT2-BiGRU


\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(7,0.11)}; %  CodeT5

%\addplot [draw=black, color=Cyan, preaction={fill, Cyan}, semithick, pattern=grid, pattern color = white]coordinates {(17,93.41)}; % DS-R1-GRU

\addplot[draw=black, color=Green, preaction={fill, Green}, semithick, pattern=grid, pattern color = white]coordinates {(8,0.11)}; % CodeT5P

%\addplot [draw=black, color=orange, preaction={fill, orange}, semithick, pattern=grid, pattern color = white] coordinates {(19,92.88)}; % DS-R1-BiLSTM

%\addplot [draw=black, color=SpringGreen, preaction={fill, SpringGreen}, semithick, pattern=grid, pattern color = white] coordinates {(20,92.45)}; % DS-R1-BiGRU



%(BERT-LSTM,91.24) (BERT-GRU,91.24) (BERT-BiLSTM,91.24) (BERT-BiGRU,91.24) (RoBERTa-base,91.32) (RoBERTa-GRU,91.68) (RoBERTa-LSTM,91.80) (RoBERTa-BiLSTM,92.36) (RoBERTa-BiGRU,92.36)







%\addplot [draw=black, semithick, pattern=north east lines, pattern color = black] coordinates {($Sorting$,26326) ($Searching$,26173) };

%\legend{$\mathbf{F1}_w$ Score, $\mathbf{A}$ Score}
\end{axis}
 


==> training_parameters.tex <==

\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    %xlabel={$minSup$},
    ylabel={Parameters (Millions)},
    ylabel near ticks, ylabel shift={-5pt},
    width=\linewidth,
    width=4.6cm,
    height=4cm,
    grid,
    grid style={gray!50},
    grid=both,
    %ymode=log,                         % <-- use log scale here
    %log basis y={10},                 % base-10 log scale
    %ymin=100, ymax=2000,             % adjust range for log scale
    %ymax=132,
    %xmin=0, xmax=13,
    %ymin=20, ymax=75,
    % xtick={0,20,40,60,80,100},
    ytick={110,115,120,125,130, 135},
    %legend style={at={(axis cs:10,60)},anchor=south east},
    symbolic x coords={RoBERTa, CodeBERT, BioLinkBERT, CodeT5, CodeT5$^+$, GPT2},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    ymajorgrids=true,
    grid style=solid,
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    legend style={at={(0.5,-0.25)},
    legend style={draw=none},
    anchor=north, legend columns=2},
]

%\addplot [mark=*, red, dashed] table[x=N,y=No_Sym] {data.dat};


\addplot[mark=otimes*, orange, solid, every mark/.append style={solid, fill=orange}]
    coordinates {
(RoBERTa,124.66)
(CodeBERT,124.65)
(BioLinkBERT,108.24)
(CodeT5,109.6)
(CodeT5$^+$,109.6)
(GPT2, 124.44)

    };
    \addlegendentry{Base}
    
\addplot[mark=square*, blue, solid, every mark/.append style={solid, fill=blue}]
    coordinates {
(RoBERTa,125.1)
(CodeBERT,125.7)
(BioLinkBERT,109.29)
(CodeT5,110.07)
(CodeT5$^+$,112.23)
(GPT2, 125.49)


    };
\addlegendentry{LSTM}

\addplot[mark=diamond*, red, solid, every mark/.append style={solid, fill=red}]
    coordinates {
(RoBERTa,129.9)
(CodeBERT,126.75)
(BioLinkBERT,113.49)
(CodeT5,110.53)
(CodeT5$^+$,111.7)
(GPT2, 126.54)
    };
\addlegendentry{BiLSTM}

\addplot[mark=*, teal, solid, every mark/.append style={solid, fill=teal}]
    coordinates {
(RoBERTa,125.43)
(CodeBERT,126.62)
(BioLinkBERT,110.21)
(CodeT5,111.58)
(CodeT5$^+$,110.4)
(GPT2, 125.23)

    };
\addlegendentry{GRU}
    
\addplot[mark=triangle*, magenta, solid, every mark/.append style={solid, fill=magenta}]
    coordinates {
(RoBERTa,128.59)
(CodeBERT,128.59)
(BioLinkBERT,112.18)
(CodeT5,113.55)
(CodeT5$^+$,111.18)
(GPT2, 126.02)

    };
\addlegendentry{BiGRU}

\end{axis}

==> training_parameters_back.tex <==

\begin{axis}[
    %title={Temperature dependence of CuSO$_4\cdot$5H$_2$O solubility},
    %xlabel={$minSup$},
    ylabel={Parameters (Hundreds of Millions)},
    ylabel near ticks, ylabel shift={-5pt},
    width=\linewidth,
    width=4.6cm,
    height=4cm,
    grid,
    grid style={gray!50},
    grid=both,
    %ymode=log,                         % <-- use log scale here
    %log basis y={10},                 % base-10 log scale
    %ymin=100, ymax=2000,             % adjust range for log scale
    %ymax=1600,
    %xmin=0, xmax=13,
    %ymin=20, ymax=75,
    % xtick={0,20,40,60,80,100},
    %ytick={110,115,120,125,130},
    %legend style={at={(axis cs:10,60)},anchor=south east},
    symbolic x coords={RoBERTa, CodeBERT, BioLinkBERT, CodeT5, CodeT5$^+$, DeepSeek-R1},
    xtick=data,
    x tick label style={rotate=25,anchor=east},
    ymajorgrids=true,
    grid style=solid,
    label style={font=\tiny},
    every node near coord/.append style={font=\tiny},
    legend style={font=\tiny},
    tick label style={font=\tiny},
    legend style={at={(0.5,-0.25)},
    legend style={draw=none},
    anchor=north, legend columns=2},
]

%\addplot [mark=*, red, dashed] table[x=N,y=No_Sym] {data.dat};


\addplot[mark=otimes*, orange, solid, every mark/.append style={solid, fill=orange}]
    coordinates {
(RoBERTa,124.66)
(CodeBERT,124.65)
(BioLinkBERT,108.24)
(CodeT5,109.6)
(CodeT5$^+$,109.6)
(DeepSeek-R1, 1543.72)

    };
    \addlegendentry{Base}
    
\addplot[mark=square*, blue, solid, every mark/.append style={solid, fill=blue}]
    coordinates {
(RoBERTa,125.1)
(CodeBERT,125.7)
(BioLinkBERT,109.29)
(CodeT5,110.07)
(CodeT5$^+$,112.23)
(DeepSeek-R1, 1545.55)


    };
\addlegendentry{LSTM}

\addplot[mark=diamond*, red, solid, every mark/.append style={solid, fill=red}]
    coordinates {
(RoBERTa,129.9)
(CodeBERT,126.75)
(BioLinkBERT,113.49)
(CodeT5,110.53)
(CodeT5$^+$,111.7)
(DeepSeek-R1, 1547.39)
    };
\addlegendentry{BiLSTM}

\addplot[mark=*, teal, solid, every mark/.append style={solid, fill=teal}]
    coordinates {
(RoBERTa,125.43)
(CodeBERT,126.62)
(BioLinkBERT,110.21)
(CodeT5,111.58)
(CodeT5$^+$,110.4)
(DeepSeek-R1, 1545.09)

    };
\addlegendentry{GRU}
    
\addplot[mark=triangle*, magenta, solid, every mark/.append style={solid, fill=magenta}]
    coordinates {
(RoBERTa,128.59)
(CodeBERT,128.59)
(BioLinkBERT,112.18)
(CodeT5,113.55)
(CodeT5$^+$,111.18)
(DeepSeek-R1, 1546.47)

    };
\addlegendentry{BiGRU}

\end{axis}
